The SuperM-Tree: Indexing metric spaces with sized objects

A common approach to implementing similarity search applications is the usage of distance functions, where small distances indicate high similarity. In the case of metric distance functions, metric index structures can be used to accelerate nearest neighbor queries. On the other hand, many applications ask for approximate subsequences or subsets, e.g. searching for a similar partial sequence of a gene, for a similar scene in a movie, or for a similar object in a picture which is represented by a set of multidimensional features. Metric index structures such as the M-Tree cannot be utilized for these tasks because of the symmetry of the metric distance functions. In this work, we propose the SuperM-Tree as an extension of the M-Tree where approximate subsequence and subset queries become nearest neighbor queries. In order to do this, we introduce metric subset spaces as a generalized concept of metric spaces. Various metric distance functions can be extended to metric subset distance functions, e.g. the Euclidean distance (on windows), the Hausdorff distance (on subsets), the Edit distance and the Dog-Keeper distance (on subsequences). We show that these examples subsume the applications mentioned above.

==> brownian.tex <==
\section{Random Accelerated Motion Generator}
\label{sec:ram}

The \ram{} generator produces classes by first generating \emph{base time series} using impulse driven motions with random acceleration (cf. Section~\ref{sec:basetimeseries} for details).
\emph{Representatives} of the classes are generated by distorting the base time series in space and time.

\subsection{Base Time Series Generator}
\label{sec:basetimeseries}

The Brownian motion is a common model of random motion in physics, for example to model movement of molecules in gases.
Basically, each next position of a molecule is obtained as a randomized position around the current position.

In order to achieve more \textit{curve like} time series, we keep an impulse vector and add that to the current position to obtain the next position.
In each step, we add a normal distributed random vector to the impulse vector.
Hence we generate series by distorting the first derivative instead of the current position.

To model edges in the generated time series, we restrict the movement to a ball with a constant radius $R$.
When the time series is about to leave the restricted area, we simply let it bounce off the sphere so the time series remains in the interior.
Algorithm~\ref{alg:velocity} provides the pseudocode for data generation and Figure~\ref{fig:velocity} shows an example for a 2-dimensional time series.
In the algorithm, \texttt{uniformBall} returns a uniform distributed vector from the interior of a union spere and \texttt{uniformSphere} returns a uniform distributed vector on a union sphere.

\begin{algorithm}
    \caption{Random Accelerated Motion Generator}
    \begin{lstlisting}
Algorithm: rambase
Input: length $l$, dimensionality $n$, radius $r$
Output: time series $s$

let $s$ be an $n$-dimensional time series of length $l$
$v = (0,\cdots,0)$
$\nu = $ normal$(0, 1)$
$s_0 = $ uniformBall$(r)$
for $i$ from $1$ to $l-1$
    $v = v\,+$ uniformSphere$(r)$
    $s_i = s_{i-1}+v$
    if $\|s_i\|_2 > r$
        // rescale $p$ to stay within the ball with radius $r$
        $s_i = s_i \cdot \frac{r}{\|p\|_2}$
        $v = $ reflect $v$ on sphere at point $p$
return $s$
    \end{lstlisting}
    \label{alg:velocity}
\end{algorithm}

\begin{figure}
    \centering
    \includegraphics[width=.49\linewidth]{images/velocity_1}
    \includegraphics[width=.49\linewidth]{images/velocity_2}
    \caption{Two examples for a random accelerated motion in 2-dimensional space.}
    \label{fig:velocity}
\end{figure}

\subsection{Generating Representatives}

We generate representatives of a class corresponding to a base time series by distorting the time series in space and time seperately.

\paragraph{Distortion in Space}

Figure~\ref{fig:ct_examples} shows examples from the character trajectories dataset \cite{UCIDatasets}.
Naturally, the representatives of a class do not match exactly.
We try to imitate this property by adding noise to the first derivative of the time series.
However, to prevent large divergence on long time series, we limit the maximum distance to the base time series by a distortion parameter.

\begin{figure}
    \centering
    \includegraphics[width=.49\linewidth]{images/ct_examples1.pdf}
    \includegraphics[width=.49\linewidth]{images/ct_examples2.pdf}
    \caption{Two time series representatives from two classes of the character trajectories dataset \cite{UCIDatasets}.}
    \label{fig:ct_examples}
\end{figure}

Hence, to distort a given time series in space, we add a standard normal distributed random vector to the first derivative of each point analogously to the base time series generator.
This also includes the first point of the time series by assuming that its predecessor is the null point $\textbf{0}=(0,\cdots,0)$.
Figure~\ref{fig:ram_spacedistortion} shows two example time series and a copy for each with distorted derivatives.

Comparing Figure~\ref{fig:ct_examples} and Figure~\ref{fig:ram_spacedistortion} shows indeed that we could imitate the properties from the character trajectories dataset.

%Given a \textit{distortion parameter} $D$, we add a random vector distributed with a multidimensional normal distribution to each element of the time series.
%The mean of the normal distribution is $\mu=0$ and $\sigma^2=\frac{D^2}{9}$ such that $99\%$ of the generated random vectors are within a ball around $0$ with radius $D$.
%If the random vector is out of the ball, we pull it back to the border.

\begin{figure}
    \centering
    \includegraphics[width=.49\linewidth]{images/velocity_1_0.pdf}
    \includegraphics[width=.49\linewidth]{images/velocity_2_0.pdf}
    \caption{Two time series (yellow) and their distorted derivative (blue); length: $100$; dimensionality: $2$; distortion: $5$ (left) and $25$ (right).}
    \label{fig:ram_spacedistortion}
\end{figure}

\paragraph{Distortion in Time}

In order to apply distortion in time we first interpret the time series as a continuous curve.
Points between two adjacent points of the time series are computed using simple linear interpolation.
Then, we reparameterize the curve in terms of the arc length instead of the time.
Finally, the time distorted time series consists of the first element of the time series, a set of points uniformly distributed on the reparameterized curve, and the last element of the time series.
Algorithm~\ref{alg:timedistortion} provides the pseudocode for the time distortion and Figure~\ref{fig:ram_timedistortion} shows two examples of time distorted time series.

\begin{algorithm}
    \caption{Time Distortion of a Time Series}
    \begin{lstlisting}
Algorithm: timedistortion
Input: time series $s$ of length $L$
Output: time series $\tilde s$

// get arc length up to each point of the time series
$\ell_i=\sum_{j=1}^{i} \|s_j-s_{j-1}\|_2$
// get uniformly distributed values along the complete arc
$t=(0,\ell_{L-1})$
repeat $L-2$ times
    $t=t\,\circ\,$uniform$([0,\ell_{L-1}])$
// interpolate between reparameterized points
$\tilde s = ()$
for $x$ in $sort(t)$
    // find correct index
    $i=\min\left\{ i\mid \ell_i \leq x < \ell_{i+1} \right\}$
    // interpolation parameter
    $u=\frac{x-\ell_i}{\ell_{i+1}-\ell_i}$
    $\tilde s = \tilde s\circ \left( \left( 1-u \right)\cdot s_i + u\cdot s_{i+1} \right)<++>$
return $\tilde s$
    \end{lstlisting}
    \label{alg:timedistortion}
\end{algorithm}

\begin{figure}
    \centering
    \includegraphics[width=.49\linewidth]{images/velocity_1_time.pdf}
    \includegraphics[width=.49\linewidth]{images/velocity_2_time.pdf}
    \caption{Two time series and their time distorted (blue) versions; length: $100$; dimensionality: $2$.}
    \label{fig:ram_timedistortion}
\end{figure}

\subsection{Dataset Generator}

As mentioned in the beginning of this section, we use the base time series generator to generate the classes.
The time distortion and space distortion algorithms generate the actual representatives of the classes.

Hence, to generate a dataset $\mathcal D$ with $C$ classes each having $N$ representatives, first call \texttt{rambase} $C$ times to generate $T_{i,0}$ ($1 \leq i \leq C$).
Then, for each $1\leq i\leq C$, call \texttt{timedistortion} and \texttt{spacedistortion} $N$ times to generate $T_{i,j}$ ($1\leq j\leq N$).
The dataset consists of each $T_{i,j}$ for $1\leq i\leq C$ and $1\leq j\leq N$.
\begin{align*}
    \mathcal C &\coloneqq \left\{ T_{i,0} = \texttt{rambase}( L, n, r ) \mid 1\leq i\leq C \right\} \\
    \mathcal R_i &\coloneqq \left\{ T_{i,j} = \texttt{spacedistortion}\big( \right. \\
                 & \quad\quad\quad\quad\quad \left. \texttt{timedistortion}( T_{i,0} ), D\big) \right\} \\
    \mathcal D &\coloneqq \bigcup_{i=1,\ldots,j} \mathcal R_i
\end{align*}
where $n$ is the desired dimensionality, $r$ is the radius of the bounding sphere, $L$ is the desired length of the time series, and $D$ the desired degree of distortion within each class.
Figure~\ref{fig:ram_full} shows two examples of a base time series and their time and space distorted representatives.

\begin{figure}
    \centering
    \includegraphics[width=.49\linewidth]{images/velocity_1_full.pdf}
    \includegraphics[width=.49\linewidth]{images/velocity_2_full.pdf}
    \caption{Two base time series and their distorted (blue) versions; length: $100$; dimensionality: $2$; radius: $75$, distortion: $5$ (left) and $25$ (right).}
    \label{fig:ram_full}
\end{figure}



==> cbf.tex <==
\section{Cylinder-Bell-Funnel}
\label{sec:cbf}

N. Saito proposed the well known 1-dimensional cylinder-bell-funnel dataset in his PhD thesis \cite{CBF}.
It is an artificial dataset consisting of three different classes of time series: cylinder, bell, and funnel.

For the time series synthesizer, let $\ell>0$ be a fixed length of the time series and $\mathcal N$ be a standard normal distributed random variable.
Furthermore, fixiate $a$ and $b$ uniformly distributed over $\left[ \ell\cdot\frac 1 8, \ell\cdot\frac 2 8 \right]$ and $\left[ \ell\cdot\frac 6 8, \ell\cdot\frac 7 8  \right]$, respectively and $\nu=6+\mathcal N$ per generated time series.
Each time series has a prefix $\mathcal P$ of length $a$ and suffix $\mathcal S$ of length $\ell-b$ containing standard normal distributed random numbers $\left( \mathcal N, \cdots, \mathcal N \right)$.

The middle parts of random \emph{cylinder} ($\mathcal C$), \emph{bell} ($\mathcal B$) and \emph{funnel} ($\mathcal F$) time series are a plateau, a rising linear function, and a falling linear function, respectively.
Their length is $b-a$, thus
\begin{align}
    \label{eq:cbf}
    \mathcal C &\coloneqq \mathcal P\times\left( \cdots, \nu+\mathcal N, \cdots \right)\times\mathcal S \\
    \mathcal B &\coloneqq \mathcal P\times\left( \cdots, \nu\cdot\frac{i-a}{b-a}+\mathcal N, \cdots \right)\times\mathcal S \\
    \mathcal F &\coloneqq \mathcal P\times\left( \cdots, \nu\cdot\frac{b-i}{b-a}+\mathcal N, \cdots \right)\times\mathcal S
\end{align}
where $\nu=6+\mathcal N$ is chosen once per time series (cf. Figure~\ref{fig:cbf} for examples).

\begin{figure}
    \centering
    \includegraphics[width=.32\linewidth]{images/cylinder}
    \includegraphics[width=.32\linewidth]{images/bell}
    \includegraphics[width=.32\linewidth]{images/funnel}
    \caption{Examples for cylinder (left), bell (center), and funnel (right) time series resp..}
    \label{fig:cbf}
\end{figure}

We canonically extend \cbf{} to generate multidimensional time series by generating one of these types for each dimension with the same starting and ending positions $a$ and $b$ (cf. Figure~\ref{fig:cbf_md} for a 2-dimensional example).
Thus, the input parameters are the length of the time series and a vector $\mathbf t$ with values $c$, $b$, and $f$ claiming which type to synthesize per dimension.
Given the dimensionality $n$, the multidimensional \cbf{} generator produces a maximum number of $3^n$ different classes, which is the set of all combinations of $c$, $b$, and $f$.

\begin{figure}
    \centering
    \includegraphics[width=.32\linewidth]{images/cb}
    \includegraphics[width=.32\linewidth]{images/cb2}
    \includegraphics[width=.32\linewidth]{images/cb1}
    \caption{An example for a 2-dimensional CBF time series (left).
    Its first dimension is a cylinder (center) and its second dimension is a bell (right).}
    \label{fig:cbf_md}
\end{figure}



==> gistImplementation.tex <==

\section{GiST Implementation}
\label{sec:gistimplementation}

\begin{itemize}
    \item Description of the GiST interface
\end{itemize}


==> synthesizers.tex <==
\input{cbf.tex}
\input{brownian.tex}

